TSGN: Temporal Scene Graph Neural Networks with Projected Vectorized Representation for Multi-Agent Motion Prediction

Predicting future motions of nearby agents is essential for an autonomous vehicle to take safe and effective actions. In this paper, we propose TSGN, a framework using Temporal Scene Graph Neural Networks with projected vectorized representations for multi-agent trajectory prediction. Projected vectorized representation models the traffic scene as a graph which is constructed by a set of vectors. These vectors represent agents, road network, and their spatial relative relationships. All relative features under this representation are both translationand rotation-invariant. Based on this representation, TSGN captures the spatial-temporal features across agents, road network, interactions among them, and temporal dependencies of temporal traffic scenes. TSGN can predict multimodal future trajectories for all agents simultaneously, plausibly, and accurately. Meanwhile, we propose a Hierarchical Lane Transformer for capturing interactions between agents and road network, which filters the surrounding road network and only keeps the most probable lane segments which could have an impact on the future behavior of the target agent. Without sacrificing the prediction performance, this greatly reduces the computational burden. Experiments show TSGN achieves state-of-the-art performance on the Argoverse motion forecasting benchmar.

==> chapters/METHOD.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\section{METHOD}\label{chapter:METHOD}
In this section, we formally introduce our proposed temporal traffic scene representation and prediction framework: THSGN.
\subsection{TEMPORAL TRAFFIC SCENE REPRESENTATION} %\label{chapter:TEMPORAL TRAFFIC SCENE REPRESENTATION}
Temporal traffic scene representation is the first step in our prediction framework. To represent the traffic scene in a form of structured graph data, we convert it into a vectorized representation. The features of road network, agents' dynamics, and the interactions among them at each timestamp are represented in a vectorized form. We adopt the feature representation of HiVT and extend it. In the remainder of this chapter, we will introduce our feature representation in a detail way. Our introduced extended features of the traffic scene and the original features of HiVT in their definitions are presented in blue and black respectively. 

%\section{Temporal Traffic Scene Representation}
%we adopt its symmetrical representation method. on the basis of it, we propose p v r  %Specifically, (the vectorized traffic scene includes)

\subsubsection{Node Feature Representation}

For traffic agents,  we extract their trajectory segments which are in a form of directed splines with respect to time. We consider each agent at each timestamp as a node and we characterize these temporal geometric nodes' attributes as $\mathbf{n}_{a} = \{\mathbf{d}^{t}_i, {\color{cyan}\mathbf{v}^{t}_i}, {\color{cyan}s^{t}_i}, {\color{cyan}\mathbf{a}^{t}_i}, {\color{cyan}\Delta t^{t}}, \mathbf{b}_i|i=1,...,N_{t}, t=0,...,19\}$ with
\begin{align}
    &\mathbf{p}^{t}_i = [x^{t}_i, y^{t}_i]\\
    &\mathbf{d}^{t}_i = \mathbf{p}^{t}_i - \mathbf{p}^{t-1}_i\\
    &\mathbf{d_x}^{t}_i = x^{t}_i - x^{t-1}_i\\
    &\mathbf{d_y}^{t}_i = y^{t}_i - y^{t-1}_i\\
    &{\color{cyan}\mathbf{v}^{t}_i} = \frac{\mathbf{d}^{t}_i}{\Delta t^{t}}\\ 
    &{\color{cyan}s^{t}_i} = \lVert {\color{cyan}\mathbf{v}^{t}_i} \rVert\\
    &\alpha^{t}_i = \arctan{\frac{\mathbf{d_y}^{t}_i}{\mathbf{d_x}^{t}_i}}\\
    &{\color{cyan}\mathbf{a}^{t}_i} = [\cos(\alpha^{t}_i),\sin(\alpha^{t}_i)]\\ 
    &{\color{cyan}\Delta t^{t}} = t^{t} - t^{t-1}
\end{align}

where $N_{t}$ represents the total number of agents at timestamp $t$, $\mathbf{p}^{t}_i$ is the location vector which consists of the lateral and longitudinal position of agent $i$ at timestamp $t$, $\mathbf{d}^{t}_i$ is the displacement vector from timestamp $t-1$ to timestamp $t$, $\mathbf{v}^{t}_i$ is the velocity, $s^{t}_i$ is the speed, $\mathbf{a}^{t}_i$ is the heading vector which consists of the cosine and sine of the agent's heading $\alpha^{t}_i$, $\Delta t^{t}$ is the timestamp difference, and $\mathbf{b}_i$ corresponds to semantic attribute, such as object type. The sampling rate is $10$Hz, but we found it deviates in different scenes, thus we include the timestamp difference into the node feature.\\  %(Besides, T is the total historical time steps)\\

For the road network, we extract the coordinates of the lane segments and their semantic attributes, such as turn direction, with or without traffic control, whether or not this lane segment is an intersection, etc. We similarly vectorize the lane segments as the vectorization for agents. The geometric node attributes of lane segments $\mathbf{n}_{l} = \{\mathbf{d}_\xi,{\color{cyan}\mathbf{a}_\xi},{\color{cyan}l_\xi},\mathbf{b}_\xi|\xi=1,...,M\}$ consist of the displacement vector $\mathbf{d}_\xi$ of each lane segment, heading vector $\mathbf{a}_\xi$, the length of the lane segment $l_\xi$, and also the semantic attribute $\mathbf{b}_\xi$, where
\begin{align}
    &\mathbf{d}_\xi = \mathbf{p}^1_\xi  - \mathbf{p}^0_\xi\\
    &{\color{cyan}\mathbf{a}_\xi} = [\cos(\alpha_\xi),\sin(\alpha_\xi)]\\ 
    &{\color{cyan}l_\xi} = \lVert \mathbf{d}_\xi \rVert
    %&\boldsymbol\ell = \{\mathbf{d}_\xi,\mathbf{a}_\xi,l_\xi|\xi=1,...,M\}\\
\end{align}

$M$ is the total number of lane segments, $\mathbf{p}^0_\xi$ and $\mathbf{p}^1_\xi$ represent the start point and end point of the lane segment $\xi$ respectively. Instead of using absolute representations, using relative representations ensure that these state quantities are not affected by coordinate translation transformations, namely translation invariance.

\subsubsection{Edge Feature Representation} %$\mathbf{e}_{aa}$ in the following way: 
The node features do not preserve relative spatial relationships. Thus, we further introduce the geometric edge attributes between agents and between agents and lane segments. We characterize the edge attributes between Agents as $\mathbf{e}_{aa} = \{\mathbf{d}^{t}_{ji}, {\color{cyan}\mathbf{v}^{t}_{ji}}, {\color{cyan}l_{ji}}, {\color{cyan}s_{ji}},{\color{cyan}\mathbf{d}^{t}_{j2i}},{\color{cyan}\mathbf{v}^{t}_{j2i}},{\color{cyan}\mathbf{a}^{t}_{j2i}}|t=0,...,19;i,j=1,...,N_t, i\neq j\}$, where\\
\begin{figure}[htbp] 
\centering
%\subfigure[]{
\includegraphics[width=8.8cm]{bilds/relative_vectorf.pdf}
\caption[Projected relative vectors]{Example of projected relative position between agents and between agents and lane segments. In the case of the figure on the left, the blue agent $i$ is defined as the target agent, $\mathbf{d}_{ji}$ is the relative position vector between agent $i$ and agent $j$, $\mathbf{d}_{j2ix}$ and  $\mathbf{d}_{j2iy}$ is the lateral and longitudinal projected relative position between agent $i$ and agent $j$. In the case of the figure on the right, $\mathbf{d}_{i2\xi}$ is the relative position vector between agent $i$ and the black lane segment $\xi$, $\mathbf{d}_{i2\xi x}$ and  $\mathbf{d}_{i2\xi y}$ is the lateral and longitudinal projected relative position between agent $i$ and lane segment $\xi$}
\label{relative_vector}
\end{figure}
\begin{align}
    % &\mathbf{e}_{aa} = \{\mathbf{d}^{t}_{ji}, {\color{cyan}\mathbf{v}^{t}_{ji}}, {\color{cyan}l_{ji}}, {\color{cyan}s_{ji}},{\color{cyan}\mathbf{d}^{t}_{j2i}},{\color{cyan}\mathbf{v}^{t}_{j2i}},{\color{cyan}\mathbf{a}^{t}_{j2i}}|t=0,...,19;i,j=1,...,N_t, i\neq j\}\\ 
    &\mathbf{d}^{t}_{ji} = \mathbf{p}^{t}_i - \mathbf{p}^{t}_j\\
    &{\color{cyan}l^{t}_{ji}} = \lVert \mathbf{d}^{t}_{ji} \rVert\\
    &{\color{cyan}\mathbf{v}^{t}_{ji}} = {\color{cyan}\mathbf{v}^{t}_i} - {\color{cyan}\mathbf{v}^{t}_j}\\
    &{\color{cyan}s^{t}_{ji}} = \lVert {\color{cyan}\mathbf{v}^{t}_{ji}} \rVert\\
    &{\color{cyan}\mathbf{d}^{t}_{j2i}} =\mathbf{R}^{t}_{i}^{\top} \mathbf{d}^{t}_{ji}\\
    &{\color{cyan}\mathbf{v}^{t}_{j2i}} = \mathbf{R}^{t}_{i}^{\top} {\color{cyan}\mathbf{v}^{t}_{ji}}\\
    &\alpha^{t}_{ji} = \alpha^{t}_{i}-\alpha^{t}_{j}\\
    &{\color{cyan}\mathbf{a}^{t}_{j2i}} = [\cos(\alpha^{t}_{ji}),\sin(\alpha^{t}_{ji})]
\end{align}\\
where $\mathbf{d}^{t}_{ij}$ is the relative position vector between agent $i$ and agent $j$ at timestamp $t$, $l^{t}_{ij}$ is the distance, $\mathbf{v}^{t}_{ij}$ is the relative velocity and $s_{ij}$ is the relative speed. $\mathbf{R}^{t}_{i}$ is the rotation matrix parameterized by the heading $\theta^t_{i}$ of the target agent $i$ at the timestamp $t$. $\mathbf{d}^{t}_{j2i}$ and $\mathbf{v}^{t}_{j2i}$ represent the projected relative position vector and projected relative velocity respectively, and $\mathbf{a}^{t}_{j2i}$ is the relative heading vector.\\

The projected relative position is defined as projecting relative position in the direction of the heading of the target agent. An example is shown in the left side of Fig. \ref{relative_vector}. In this case, the blue agent $i$ is defined as the target agent, $\mathbf{d}^{t}_{ij}$ is the relative position between agent $i$ and agent $j$, $\mathbf{d}^{t}_{j2ix}$ and $\mathbf{d}^{t}_{j2iy}$ are the lateral and longitudinal projected relative position between agent $i$ and agent $j$. Similarly, we obtain the projected relative velocity by projecting relative velocity in the direction of the heading of the target agent. \\

We characterize the edge features between agents and lane segments as $\mathbf{e}_{al} = \{\mathbf{d}^{t}_{i\xi}, {\color{cyan}\mathbf{d}^{t}_{i2\xi}},{\color{cyan}l^{t}_{i\xi}},{\color{cyan}\mathbf{v}^{t}_{i2\xi}},{\color{cyan}\mathbf{a}^{t}_{i2\xi}}|t=0,...,19; i=1,...,N_t;\xi==1,...,M\}$, where
\begin{align}
    % &\mathbf{e}_{al} = \{\mathbf{d}^{t}_{i\xi}, {\color{cyan}\mathbf{d}^{t}_{i2\xi}},{\color{cyan}l^{t}_{i\xi}},{\color{cyan}\mathbf{v}^{t}_{i2\xi}},{\color{cyan}\mathbf{a}^{t}_{i2\xi}}\\&|t=0,...,19; i=1,...,N_t;\xi==1,...,M\}\\
    &\mathbf{d}^{t}_{i\xi} = \mathbf{p}^0_\xi - \mathbf{p}^{t}_i\\
    &{\color{cyan}\mathbf{d}^{t}_{i2\xi}} = \mathbf{R}^{t}_{\xi}^{\top} \mathbf{d}^{t}_{i\xi}\\
    &{\color{cyan}l^{t}_{ij}} = \lVert {\color{cyan}\mathbf{d}^{t}_{i\xi}} \rVert\\
    &{\color{cyan}\mathbf{v}^{t}_{i2\xi}} = \mathbf{R}^{t}_{\xi}^{\top} {\color{cyan}\mathbf{v}^{t}_{i}}\\
    &\alpha^{t}_{i\xi} = \alpha^{t}_{\xi}-\alpha^{t}_{i}\\
    &{\color{cyan}\mathbf{a}^{t}_{i2\xi}} = [\cos(\alpha^{t}_{i\xi}),\sin(\alpha^{t}_{i\xi})]
\end{align}\\
where $\mathbf{d}^{t}_{i\xi}$ is the relative position vector between agent $i$ and lane segment $\xi$ at timestamp $t$, $l^{t}_{i\xi}$ is the distance and $\mathbf{R}_{\xi}$ is the rotation matrix parameterized by the heading $\theta_{\xi}$ of the target lane. $\mathbf{d}^{t}_{i2\xi}$ and $\mathbf{v}^{t}_{i2\xi}$ represent the projected relative position vector and projected relative velocity respectively, and $\mathbf{a}^{t}_{i2\xi}$ is the relative heading vector. The projected relative position between lane segment $\xi$ and agent $i$ is defined as projecting relative position in the direction of the heading of the target lane segment $\xi$. An example is shown in the right side of the Fig. \ref{relative_vector}. In this case, $\mathbf{d}_{i2\xi}$ is the relative position vector between agent $i$ and lane segment $\xi$, $\mathbf{d}_{i2\xi x}$ and $\mathbf{d}_{i2\xi y}$ are the lateral and longitudinal projected relative position between agent $i$ and lane segment $\xi$. Similarly, we obtain the projected relative velocity $\mathbf{v}^{t}_{i2\xi}$ by projecting the agent's velocity in the direction of the heading of the target lane segment.\\

The projected relative position and the projected relative velocity depict how close two individual nodes are and how fast one node moves towards another node in both lateral and longitudinal directions. Compared to the relative representation, the projected relative representation describes the interaction between entities in a more detailed way, allowing downstream networks to better understand their behavior. Moreover, such a projected relative representation guarantees not only translation invariance but also rotation invariance naturally.\\


\subsection{PREDICTION FRAMEWORK} %\label{chapter:PREDICTION FRAMEWORK}
We introduce our prediction framework THSGN which consists of a local encoder, a global encoder, and a multimodal future decoder as well as the components of the local encoder, i.e., agent-agent transformer, agent-lane transformer, and temporal transformer. Following that, we cover details about our proposed Hierarchical Lane Transformer that let the model efficiently calculates the interactions between agents and lane segments.\\
\begin{figure*}[htbp]
\centering
%\subfigure[]{
\includegraphics[width=14cm]{images/framework1.pdf}
\caption{Overall Framework \cite{zhou2022hivt}}
\label{Overall Framework} 
\end{figure*}
\subsubsection{Temporal Hierarchical Scene Graph Neural Networks}
Based on the symmetrical representation and the local-global mechanisms of HiVT, we propose an optimized prediction framework: THSGN. An overview is shown in Fig. \ref{Overall Framework}. Firstly, the traffic scene at each timestamp is divided into a set of local regions, each corresponding to one agent and centered on it. The local region is defined as the set of all traffic entities in the receptive field, where the receptive field is the area within the radius threshold of the central agent. We employ an improved local encoder to extract agents’ spatial-temporal features from their associated local regions and a global encoder to capture long-range dependencies and interactions among local regions. Finally, the decoder outputs multimodal trajectories for multiple agents simultaneously.\\

\paragraph{Local Encoder} %{\rm AA}_{a}
%By limiting the radius of the local regions, we reduce the computational complexity of Agent-Agent Transformer and Agent-Lane Transformer, thus 
The local encoder operates the temporal scene graph in two stages. In the first stage, it models the agent-agent interactions and agent-lane interactions per time step and uses a temporal transformer module to capture the temporal dependencies across traffic scenes. Since the number of agent-lane edges is large, modeling agent-lane interactions for every timestamp suffers from the computational burden. We use a reduced receptive field of view in this stage for efficiency. In the second stage, it uses the refreshed agents' features to update the relative spatial relationships between entities and models the agent-agent interaction per time step again, followed by a temporal transformer with a classification token for summarizing the temporal information and an agent-lane transformer only focusing on the current timestamp with a larger receptive field, we obtain the final updated features for each agent. In summary, the local encoder of THSCN contains the following modules: Agent-Agent Transformer in the first stage (${\rm AA}_{a1}$) and second stage (${\rm AA}_{a2}$), Agent-Lane Transformer in the first stage (${\rm AL}_{a}$ for all timestamp) and second stage (${\rm AL}_{c}$ only for the current timestamp), and Temporal Transformer in the first stage (${\rm Temporal}_{1}$) and second stage (${\rm Temporal}_{2}$). An overview of the local encoder is shown in Fig. \ref{Local_Encoder}. In the remainder of this section, we first describe the Agent-Agent Transformer, Agent-Lane Transformer, and Temporal Transformer separately, and then we detail how these transformers are going to be used in the two different stages.


\begin{figure*}[htbp]
\centering
%\subfigure[]{
\includegraphics[width=14cm]{images/le.pdf}
\caption{Local Encoder}
\label{Local_Encoder}
\end{figure*}
\subparagraph{Agent-Agent Transformer}

% \begin{align}
%     &\mathbf{q}^{t}_i = \mathbf{W}^{Q^{space}}\mathbf{z}^{t}_i\\
%     &\mathbf{k}^{t}_{ij} = \mathbf{W}^{K^{space}}\mathbf{z}^{t}_{ij}\\
%     &\mathbf{v}^{t}_{ij} = \mathbf{W}^{V^{space}}\mathbf{z}^{t}_{ij}
% \end{align}

% \begin{align}
%     &\bm{\alpha}^{t}_i = \mathbf{W}^{Q^{space}}\mathbf{z}^{t}_i\\
%     &\mathbf{k}^{t}_{ij} = \mathbf{W}^{K^{space}}\mathbf{z}^{t}_{ij}\\
%     &\mathbf{v}^{t}_{ij} = \mathbf{W}^{V^{space}}\mathbf{z}^{t}_{ij}
% \end{align}

% \begin{align}
%     % &\bm{\alpha}^{t}_i = softmax(\frac{\mathbf{q}^{t}_i}{\sqrt{d_k}}[\{\mathbf{k}^{t}_{ij}\}_{j\in \mathcal N_{i}}]) 
%     % &\bm{\alpha}^{t}_i =  \rm{softmax}\Bigg (\frac{{\mathbf{q}^{t}_i}^{\top}}{\sqrt{d_k}} \cdot \Big [\{\mathbf{k}^{t}_{ij}\}_{j\in \mathcal N_{i}}\Big ] \Bigg) \\
%     &\bm{\alpha}^{t}_{ij} =  \rm{softmax}\Bigg (\frac{{\mathbf{q}^{t}_i}^{\top}}{\sqrt{d_k}} \cdot \mathbf{k}^{t}_{ij}\Bigg) \\
%     &\mathbf{m}^{t}_{i} = \sum_{j\in \mathcal N_{i}}\bm{\alpha}^{t}_{ij}\mathbf{v}^{t}_{ij}\\
%     &\mathbf{g}^{t}_{i} =  \rm{sigmoid}(\mathbf{W}^{ \rm{gate}}[\mathbf{z}^{t}_{i},\mathbf{m}^{t}_{i}])\\
%     &\hat{\mathbf{z}}^{t}_{i} = \mathbf{g}^{t}_{i}\odot\mathbf{W}^{ \rm{self}}\mathbf{z}^{t}_{i}+(1-\mathbf{g}^{t}_{i})\odot\mathbf{m}^{t}_{i}
% \end{align}

% \begin{align}
%    &\mathbf{Q}_{i} = \mathbf{S}_{i}\mathbf{W}^{Q^{time}}\\
%    &\mathbf{K}_{i} = \mathbf{S}_{i}\mathbf{W}^{K^{time}}\\
%    &\mathbf{V}_{i} = \mathbf{S}_{i}\mathbf{W}^{V^{time}}\\
%    &\hat{\mathbf{S}}_{i} = \rm{softmax}\Bigg (\frac{{\mathbf{Q}_i}{\mathbf{K}^{\top}_i}}{\sqrt{d_k}} + \mathbf{M}\Bigg)\mathbf{V}_{i} \\
% \end{align}

% \begin{equation*}
% \mathbf{M}_{uv} = \begin{cases}
%  -\infty &\text{if u<v}\\
% 0 &\text{otherwise}\\
% \end{cases}
% \end{equation*}

% \begin{equation}
% \begin{aligned}
% ;
% \end{aligned}           
% \end{equation}
% @
Every agent has its own pattern, they move with different trajectories and have different goals. They adjust their trajectories by implicitly inferring about the behavior of surrounding agents. These surrounding agents in turn are also influenced by their immediate neighbors and could alter their behavior over time.\\

To accurately predict the future behavior of agents in the traffic scene, we need a model to learn and understand the interactions between agents. We use a multi-head cross-attention block to learn the interaction relationships and the importance of the influence of different surrounding agents on the center agent for each local region at each time step.\\ 

Specifically, firstly, we rotate all translation-invariant but not rotation-invariant local vectors according to the heading $\theta^{T}_{i}$ of central agent $i$ at the current timestamp $T$ and apply Multi-Layer Perceptrons (MLPs) on its node attributes and edge attributes, then we 
obtain the central agent $i$'s temporal node embedding $\mathbf{z}^t_i$ and any of its associated temporal edge embedding $\mathbf{z}^t_{ij}$ which is connected with neighboring agent $j$: 
\begin{align}
    &\mathbf{z}^{t}_{i} = \phi_{\rm{center}}\Big([\mathbf{R}^{\top}_{i}\mathbf{d}^{t}_i, \mathbf{R}^{\top}_{i}{\color{cyan}\mathbf{v}^{t}_i}, \mathbf{R}^{\top}_{i}{\color{cyan}\mathbf{a}^{t}_i}, {\color{cyan}s^{t}_i}, {\color{cyan}\Delta t^{t}}, \mathbf{b}_{i}] \Big)\\
    &\mathbf{z}^{t}_{ij} = \phi_{\rm{nbr}}\Big([\mathbf{R}^{\top}_{i}\mathbf{d}^{t}_{j}, \mathbf{R}^{\top}_{i}\mathbf{d}^{t}_{ij}, \mathbf{R}^{\top}_{i}{\color{cyan}\mathbf{v}^{t}_{ij}}, {\color{cyan}l^{t}_{ij}}, {\color{cyan}s^{t}_{ij}}, {\color{cyan}\mathbf{d}^{t}_{j2i}}, {\color{cyan}\mathbf{v}^{t}_{j2i}}, {\color{cyan}\mathbf{a}^{t}_{j2i}}, \mathbf{b}_{j}] \Big)
    %\mathbf{p}^{t}_{j}-\mathbf{p}^{t-1}_{j}
    %&\mathbf{e_a} = \{\mathbf{d}^{t}_{ij}, \mathbf{v}^{t}_{ij}, l_{ij}, s_{ij},\mathbf{d}^{t}_{j2i},\mathbf{v}^{t}_{j2i},\mathbf{a}^{t}_{j2i}|t=0,...,19;i,j=1,...,N\}\\  
\end{align}
where $\phi_{\rm{center}}$ and $\phi_{\rm{nbr}}$ are MLP blocks and $\mathbf{R}^{T}_{i}$ is the rotation matrix parameterized by the heading $\theta^{T}_{i}$.
After rotation transformation, both node and edge attributes are translation and rotation invariant, their embeddings also inherit these properties. We then encode the central agent $i$'s node embedding $\mathbf{z}^t_i$ and its associated edge embedding $\mathbf{z}^t_{ij}$ by learnable matrices to obtain the query, key, and value vectors:
\begin{align}
    &\mathbf{q}^{t}_i = \mathbf{W}^{Q^{space}}\mathbf{z}^{t}_i\\
    &\mathbf{k}^{t}_{ij} = \mathbf{W}^{K^{space}}\mathbf{z}^{t}_{ij}\\
    &\mathbf{v}^{t}_{ij} = \mathbf{W}^{V^{space}}\mathbf{z}^{t}_{ij}
\end{align}
where $\mathbf{W}^{Q^{space}}$, $\mathbf{W}^{K^{space}}$, and $\mathbf{W}^{V^{space}}$ are the query, key, and value matrix for linear transformation. The cross attention block receives query $\mathbf{q}^{t}_i$, key $\mathbf{k}^{t}_{ij}$ and value $\mathbf{v}^{t}_{ij}$ as inputs, and performs the scaled  dot-product attention with a gating function $\mathbf{g}^{t}_{i}$ as:
% where $\mathbf{W}^{Q^{space}}$, $\mathbf{W}^{K^{space}} and $\mathbf{W}^{V^{space}} are the learnable matrices  query, key and value vectors respectively. (查看attention 说明，sca;ed.dot production attention)
%\begin{align}
%     &\bm{\alpha}^{t}_i = \mathbf{W}^{Q^{space}}\mathbf{z}^{t}_i\\
%     &\mathbf{k}^{t}_{ij} = \mathbf{W}^{K^{space}}\mathbf{z}^{t}_{ij}\\
%     &\mathbf{v}^{t}_{ij} = \mathbf{W}^{V^{space}}\mathbf{z}^{t}_{ij}
% \end{align}
\begin{align}
    % &\bm{\alpha}^{t}_i = softmax(\frac{\mathbf{q}^{t}_i}{\sqrt{d_k}}[\{\mathbf{k}^{t}_{ij}\}_{j\in \mathcal N_{i}}]) 
    &\bm{\alpha}^{t}_i =  \rm{softmax}\Bigg (\frac{{\mathbf{q}^{t}_i}^{\top}}{\sqrt{d_k}} \cdot \Big [\{\mathbf{k}^{t}_{ij}\}_{j\in \mathcal N_{i}}\Big ] \Bigg) \\
    &\mathbf{m}^{t}_{i} = \sum_{j\in \mathcal N_{i}}\bm{\alpha}^{t}_{ij}\mathbf{v}^{t}_{ij}\\
    &\mathbf{g}^{t}_{i} =  \rm{sigmoid}(\mathbf{W}^{ \rm{gate}}[\mathbf{z}^{t}_{i},\mathbf{m}^{t}_{i}])\\
    &\hat{\mathbf{z}}^{t}_{i} = \mathbf{g}^{t}_{i}\odot\mathbf{W}^{ \rm{self}}\mathbf{z}^{t}_{i}+(1-\mathbf{g}^{t}_{i})\odot\mathbf{m}^{t}_{i}
\end{align}
where $d_k$ is the dimensionality of the query and key and $\mathcal N_{i}$ represents the surrounding agents of agent $i$. We further apply an MLP block in conjunction with residual connections \cite{he2016deep} and takes $\hat{\mathbf{z}}^{t}_{i}$ as input to obtain the first updated node embedding $\mathbf{s}^{t}_{i}$ of agent $i$ at timestamp $t$ which incorporates interactions between agents.

\subsubsection{Agent-Lane Transformer}
The road network plays a crucial role in motion predictions. Every agent has an implicit goal, we cannot know their intentions ahead of time. However, the surrounding road network can indicate the future driving trajectories of the agents to a certain degree. To capture these implicit interactions between agents' trajectories and lane segments, we employ another multi-head cross-attention block to model these interactions. Similar to the agent-agent transformer module, according to the heading $\theta_i$ of central agent $i$,  we rotate the local lane segments, and their associated rotation-variant temporal edge attributes which are connected with the central agent $i$, and encode them by an MLP block $\phi_{\rm{lane}}$ to obtain the edge embedding between agent $i$ and lane segment $\xi$:
\begin{align}
    &\mathbf{z}_{i\xi} = \phi_{\rm{lane}}\Big([\mathbf{R}^{\top}_{i}(\mathbf{d}_{\xi}),\mathbf{R}^{\top}_{i}(\mathbf{d}_{i\xi}),{\color{cyan}\mathbf{d}_{i2\xi}}, {\color{cyan}l_{i\xi}},{\color{cyan}\mathbf{v}_{i2\xi}}, {\color{cyan}\mathbf{a}_{i2\xi}}, \mathbf{b}_{\xi}] \Big)
\end{align}

Following that, we employ the multi-head cross-attention block that takes agent $i$'s node embedding $\mathbf{s}^{t}_{i}$ as query, the edge embedding $\mathbf{z}_{i\xi}$ between central agent $i$ and lane segment $\xi$ as key and value, and performs the scaled dot-product attention the same way as the agent-agent transformer module, followed by an MLP block in conjunction with residual connections. We then obtain the updated node embedding $\widetilde{\mathbf{s}}^{t}_{i}$ which incorporates interactions between agents and interactions between agents and lane segments.

%summarizes spatial features of the local regions.
%node embedding 

%By moduling the agent-agent and agent-lane interaction, we obtain the spatial node embedding $\mathbf{s}^{t}_{i}$ of agent $i$ at timestamp $t$. %which incorperates interactions between agents and between agents and lanes.

% @todo, 变量名

% in practice we set the radius $d = 20$

\paragraph{Temporal Transformer} 
Historical information plays a crucial role in inferring traffic agents' dynamics in the future. We treat the encoded traffic scene at each timestamp as a whole and use a temporal transformer to capture temporal dependencies of all historical encoded traffic scenes. Specifically, we add the learnable positional embeddings \cite{vaswani2017attention} to the central agent $i$'s node embedding $\{\widetilde{\mathbf{s}}^{t}_{i}\}^{T}_{t=1}$ at each timestamp, stack them into a matrix $\widetilde{\mathbf{S}}_{i}$, and perform multi-head self-attentiondot with an MLP block $\phi_{\rm{temp}}$ as: %
\begin{align}
   &\mathbf{Q}_{i} = \widetilde{\mathbf{S}}_{i}\mathbf{W}^{Q^{time}}\\
   &\mathbf{K}_{i} = \widetilde{\mathbf{S}}_{i}\mathbf{W}^{K^{time}}\\
   &\mathbf{V}_{i} = \widetilde{\mathbf{S}}_{i}\mathbf{W}^{V^{time}}\\
   %&\hat{\mathbf{S}}_{i} = \phi_{\rm{temp}}\Bigg (\rm{softmax}\Bigg (\frac{{\mathbf{Q}_i}{\mathbf{K}^{\top}_i}}{\sqrt{d_k}}\Bigg)\mathbf{V}_{i}\Bigg)
   &\hat{\mathbf{S}}_{i} = \phi_{\rm{temp}}\Bigg (\rm{softmax}\Bigg (\frac{{\mathbf{Q}_i}{\mathbf{K}^{\top}_i}}{\sqrt{d_k}} + \mathbf{M}\Bigg)\mathbf{V}_{i}\Bigg)\\
   &\mathbf{M}_{uv} = \begin{cases}
                     -\infty &\text{if u<v and first stage}\\
                    0 &\text{otherwise}\\
                    \end{cases}
\end{align} 
where \mathbf{W}^{Q^{time}}$, $\mathbf{W}^{K^{time}}$ and $\mathbf{W}^{V^{time}}$ are the query, key and value matrix for linear transformation. $\mathbf{M}$ is the temporal mask which is used to make the tokens only focus on the preceding timestamps. The output of the temporal transformer $\hat{\mathbf{S}}_{i}$ summarizes the spatial-temporal features of agent $i$ for every timestamp.

 %By sequentially modeling agent-agent interactions, agent-lane interactions and temporal dependencies (transformer), we obtain the spatial-temporal node embedding $\mathbf{s}^{t}_{i}$ of agent $i$. %which incorperates interactions between agents and between agents and lanes.


% (... (Unlike other methods,)
% Specifically, firstly, similar to BERT, ..
% we extand the embeddings with an extra learnable token 
% sT +1 ∈ Rdh to the end of the input sequence. This token is used as the aggregate sequence representation for classification
% tasks. (classify different manuevers of agents)

% #equ..  +learnable token, positonal embeddings.. ()
% %%#看BERT怎么写
% its input representation of temporal transformer $S$ is
% constructed by summing the embeddings(), and positional embeddings.
% To obtain temporal dependent scene features, we compute the self attention of $S$:


% @
% expect the hidden states of an LSTM
% to capture these time varying motion-properties.

% #
% Agent history encoding. The agent history encoding is obtained by concatenating the output of three sources:

% 3. MCG blocks applied to the set of history elements. Each element in the set consists of a historical position and


% where the second argument is the input context vector to MCG, which in this case is a concatenation of the modeled
% agent’s history embedding, and the AV’s interaction embedding

% @is the temporal mask that
% enforces the tokens only attend to the preceding time steps.
% We don't (@看Scene transformer 怎么写)
%Citation test~\parencite{latex}. and  \parencite{ngiam2021scene}
\subsubsection{First Stage}
In the first stage, the local encoder models the agent-agent interactions and agent-lane interactions per time step. These two interaction modules aggregate the spatial information of the temporal traffic scene for every timestamp. As explained before, due to the great computational complexity, we use a reduced receptive field of view in this stage for efficiency. Taking the encoded temporal traffic scene as input, the temporal transformer further summarizes the temporal information. Unlike most approaches which only capture the temporal dependencies of agents' historical dynamics, we propose to incorporate the agent-agent interactions and agent-lane interactions to update agents' node embedding for every timestamp, since the interactions in the past will affect the agents' pattern in the future. Through these operations, we obtain updated node embeddings for every agent which summarizes the spatial-temporal information of the temporal traffic scene. 

\subsubsection{Second Stage}
% To summarize the whole temporal sequence into one single token. It is very important to explain the idea and justification behind your choices rather than just describing them technically which can be hard to understand,

% receptive field. Explain what this is and why. You don't even explain that the field was restrained in the first step.]
\label{sec:Second Part}
In the second stage, we use the refreshed node embeddings of agents in the first stage to update the edge embeddings between agents as: %and between agents and lanes as following:
\begin{align}
    %&\mathbf{z}^{t}_{i} = \phi_{\rm{center}}\Big([\mathbf{R}^{T}_{i}\mathbf{d}^{t}_i, \mathbf{R}^{T}_{i}\mathbf{v}^{t}_i, \mathbf{R}^{T}_{i}\mathbf{h}^{t}_i, s^{t}_i, \Delta t^{t}, \mathbf{a}_{i}] \Big)\\
    &\mathbf{z}^{t}_{{ij}_{2}} = \phi_{\rm{nbr}_2}\Big([\hat{\mathbf{s}}^{t}_{i},\mathbf{z}^{t}_{ij}] \Big)
    %&\mathbf{z}_{{i\xi}_{2}} = \phi_{\rm{lane}_2}\Big([\mathbf{s}^{t}_{i},\mathbf{z}_{{i\xi}] \Big)
\end{align}

where $\{\hat{\mathbf{s}}^{t}_{i}\}^{T}_{t=1}$ is the unstacked result of $\hat{\mathbf{S}}_{i}$. We then use the refreshed agents’ nodes embeddings $\{\hat{\mathbf{s}}^{t}_{i}\}^{T}_{t=1}$ and edges embeddings between agents $\mathbf{z}^{t}_{{ij}_{2}}$ to repeat an agent-agent interaction encoding for every timestamp. In the first modeling of agent-agent interactions, the agents lacked information about the road network, which could in turn affect their behaviors and interactions. Thus, we apply it again, after all agents are incorporated with the road network information. Afterwards, we apply another temporal transformer with an extra learnable classification token \cite{devlin2018bert} and a temporal mask $\mathbf{M}$ to summarize the whole temporal sequence into one single token $\bar{\mathbf{s}}_{i}$.\\

% that enforces the tokens only attend to the preceding time steps:
% \begin{align}
%     &\hat{\mathbf{S}}_{i} = \rm{softmax}\Bigg (\frac{{\mathbf{Q}_i}{\mathbf{K}^{\top}_i}}{\sqrt{d_k}} + \mathbf{M}\Bigg)\mathbf{V}_{i}\\
%     &\mathbf{M}_{uv} = \begin{cases}
%                      -\infty &\text{if u<v}\\
%                     0 &\text{otherwise}\\
%                     \end{cases}
% \end{align}
The edge embeddings between agents and lane segments are calculated as: 
\begin{align}
    &\mathbf{z}_{{i\xi}_{2}} = \phi_{\rm{lane}_2}\Big([\bar{\mathbf{s}}_{i},\mathbf{z}_{i\xi}]\Big)
\end{align}
We input the updated extra classification token $\bar{\mathbf{s}}_{i}$ as query and updated edge embeddings $\mathbf{z}_{{i\xi}_{2}}$ between agent $i$ and lane segment $\xi$ as key and value to another same agent-lane interaction module with a larger receptive field. We obtain the final node embedding $\mathbf{h}_{i}$ of the central agent $i$. $\mathbf{h}_{i}$ summarizes the fused rich spatial-temporal features of the agent $i$. It incorporates agent $i$'s dynamics and the iterative interactions between agent $i$ and its surrounding environment. The final local representation for all agents $\mathbf{h}$ is defined as $\mathbf{h} = \{\mathbf{h}_i|i=1,...,N\}$, where $N$ is the number of agents.

\subsection{Global Interaction Module}
The local encoder output represents the features of the central agent within its local region, but it does not incorporate the pairwise interactions between local regions and lack the long-range dependencies in the scene. To address these issues, we apply a global interaction module \cite{zhou2022hivt} for high-order interactions.\\

Similar to the Agent-Agent Transformer, we use an MLP $\phi_{rel}$ to obtain the edge embedding $\mathbf{g}_{ij}$ between agent $i$'s and agent $j$'s local regions:

\begin{align}
    &\mathbf{g}_{ij} = \phi_{\rm{rel}}\Big([\mathbf{R}^{\top}_{i}\mathbf{d}^{T}_{ij}, \mathbf{R}^{\top}_{i}{\color{cyan}\mathbf{v}^{T}_{ij}}, {\color{cyan}l^{T}_{ij}}, {\color{cyan}s^{T}_{ij}}, {\color{cyan}\mathbf{d}^{T}_{j2i}}, {\color{cyan}\mathbf{v}^{T}_{j2i}}, {\color{cyan}\mathbf{a}^{T}_{j2i}]} \Big)
\end{align}

where $T$ represents the last current timestep. We take the local node embedding $\mathbf{h}_i$ as query, the concatenation of $\mathbf{h}_j$ and $&\mathbf{z}_{ij}$ as key and value:
\begin{align}
    & \widetilde{\mathbf{q}}_i = \mathbf{W}^{Q^{global}}\mathbf{h}_i\\
    & \widetilde{\mathbf{k}}_{ij} = \mathbf{W}^{K^{global}}[\mathbf{h}_j,\mathbf{g}_{ij}]\\
    & \widetilde{\mathbf{v}}_{ij} = \mathbf{W}^{V^{global}}[\mathbf{h}_j,\mathbf{g}_{ij}]
\end{align}

where $\mathbf{W}^{Q^{global}}$, $\mathbf{W}^{K^{global}}$, and $\mathbf{W}^{V^{global}}$ are query, key, and value matrices for linear transformation. A  multi-head cross-attention block takes them as input and outputs agent $i$'s updated node embedding which incorporates global scene information. Afterwards, we employ an MLP block to map the updated node embedding of each agent to the final global representation $\widetilde{\mathbf{h}}$ with shape $[F, N, D]$, where $F$ is the number of mixture components, representing the multimodality of agents' trajectories in the future, $N$ is the number of agents, and $D$ is the number of agents' features. 

% $\widetilde{\mathbf{h}}_i$ with shape $[1,1,D]$ to $\widetilde{\mathbf{h}}_{Fi}$ with shape $[F, N, D]$. $N$,$F$..$\widetilde{\mathbf{h}}_i$ 
% $\widetilde{\mathbf{h}}_{Fi}$ represents the global representations for all 

%To address this issue, we introduce a mixture density network to output 

\subsection{Multimodal Future Decoder}
% [Why is there already F here ? Why do ~h and h not have the same shape ?
% This is not clear. Better explained with the resulting shape as you do afterwards
% Specify output shape after that]

In a complex traffic scene, agents behave multimodally, for example, an agent could go straight, turn left, turn right, etc., at the intersection. To characterize this phenomenon of agents, we apply a mixture density network \cite{bishop1994mixture} with GRU \cite{cho2014properties} as the decoder to output multimodal trajectories for each agent. \\

%, where $F$ is the number of mixture components, $N$ is the number of agents, $D$ is the number of agents' features and 
% based solely on the past observations of the target agent's dynamics and its surrounding environment, we can not accurately predict its future maneuver. 
%The decoder receives 
Specifically, we tile the global representation $\widetilde{\mathbf{h}}$ with shape $[F, N, D]$ and the local representation $\mathbf{h}$ with shape $[N, D]$ $H$ and $F$ time, then we obtain the tiled global representation with shape $[H, F \times N, D]$ and the tiled local representation with shape $[1, F \times N, D]$, where $H$ is the number of future steps. The GRU receives the tiled global representation as inputs and the tiled local representation as the initial hidden state and outputs $\mathbf{o}$ with shape $[H, F \times N, D]$. We further transpose the first dimension and second dimension of GRU output $\mathbf{o}$ and apply two different MLP blocks $\phi_{\rm{loc}}$, $\phi_{\rm{unc}}$ which take the GRU output $\mathbf{o}$ as input and output locations $\bm{\mu}$ with shape $[F, N, H, 2]$ and the associated uncertainty $\mathbf{b}$ with shape $[F, N, H, 2]$. We apply another MLP block $\phi_{\rm{prob}}$ with the concatenation of $\mathbf{h}$ and $\widetilde{\mathbf{h}}$ as input to obtain the probability $\bm{\pi}$ of possible future trajectories of all agents:

\begin{align}
    &\mathbf{o} = \rm{GRU}([\widetilde{\mathbf{h}}, \mathbf{h}])\\
    &\bm{\mu} = \phi_{\rm{loc}}(\mathbf{o})\\
    &\mathbf{b} = \phi_{\rm{unc}}(\mathbf{o})\\
    &\bm{\pi} = \phi_{\rm{prob}}([\widetilde{\mathbf{h}}, \mathbf{h}])
\end{align}

%  and output the 

% µt i;f 2 R2 and
% its associated uncertainty bt i;f 2 R2 of the agent per future time step in the local coordinate frame. 

% a mixture model is a probabilistic model for representing the presence of . Formally a mixture model corresponds to the mixture distribution that represents the probability distribution of observations in the overall population. 

% #todo Each traffic agent can have F distinct futures, their motions are inherently multimodal.

% The future motions of traffic agents are inherently multimodal. Thus, we parameterize the distribution of future trajectories as a mixture model where each mixture component is a Laplace distribution. The predictions are made for all
% agents in a single shot.

% @
% For each agent $i$ and each component $f$, we tile its global and local representations $F$ and $N$ time respectively. 


% The gru receives the tiled global representations with shape [H, F x N, D] as inputs and the tiled local representations with shape [1, F x N, D] as the initial hidden state and output the location µt i;

% a GRU[] receives the local and the global representations as inputs and the initial hidden state and outputs the location µt i;f 2 R2 and
% its associated uncertainty bt i;f 2 R2 of the agent per future time step in the local coordinate frame. Specifically, we expand the which have the shape of [H, F x N, D]. repeat the local representations which have the shape of [1, F x N, D]

% The output tensor of the regression head has the shape of [F; N; H; 4], where F is the number of mixture components, N is the number of
% agents in the scene, and H is the number of predicted future
% time steps. We also use another MLP followed by a softmax
% function to produce the mixing coefficients of the mixture
% model for each agent, which have the shape of [N; F].

% In order to allow the decoder to output F distinct futures, we perform
% the following operations. The decoder receives as input a tensor of shape [A; T; D] corresponding to
% A agents across T time steps and D feature dimensions. The following series of simple operations
% restructures the representation to predict F futures. First, the representation is tiled F times to
% generate [F; A; T; D]. For computational
% simplicity, the resulting representation is propagated through a small MLP to produce a return a
% tensor of the shape [F; A; T; D].

\subsection{Loss Function}
According to our observations, the tracking data of Argoverse dataset $1$ contains some noisy samples. Compared to Gaussian negative log-likelihood loss, Laplace negative log-likelihood loss is more robust to outliers, thus we design the multimodal future decoder in that way so that it predicts a parameterization of the location and its associated uncertainty corresponding to a Laplace distribution \cite{meyer2020learning}. We use the winner-take-all strategy, and only apply the loss to the best-predicted trajectory which is defined as the one that has the minimum endpoint error. Our final loss consists of the regression loss $\mathcal{L}_{\rm{reg}}$ and the classification loss $\mathcal{L}_{\rm{cls}}$:
\begin{align}
    &\mathcal{L}_{reg} = -\frac{1}{NH}\sum^N_{i=1}\sum^{T+H}_{t=T+1}\log P\Big(\mathbf{R}^{T}_{i}(\mathbf{p}^{t}_{i}-\mathbf{p}^{T}_{i}) | \hat{\bm{\mu}}^{t}_{i},\hat{\mathbf{b}}^{t}_{i}\Big)\\
    &\overline{\bm{\pi}}_{i}={\rm softmax}\Big(-\sum^{T+H}_{t=T+1}\lVert {\bm{\mu}}^{t}_{i},\mathbf{R}^{T}_{i}(\mathbf{p}^{t}_{i}-\mathbf{p}^{T}_{i}) \lVert \Big) \\
    &\mathcal{L}_{cls} = {\sum^N_{i=1}}{\rm CEL}(\overline{\bm{\pi}}_{i}, \hat{\bm{\pi}}_{i})\\
    &\mathcal{L}_{cls} = -\frac{1}{N}\sum^N_{i=1}\log\Big(sum^K_{k=1}\hat{\bm{\pi}}_{ik} \Big)\\
    &\mathcal{L}=\mathcal{L}_{\rm{reg}} + \mathcal{L}_{\rm{cls}}
\end{align}
% We parameterize the distribution of agent's future trajectory as a Laplace distribution. 

The loss function $\mathcal{L}$ consists of the regression loss $\mathcal{L}_{\rm{reg}}$ and $\mathcal{L}_{\rm{cls}}$. $\hat{\bm{\mu}}^{t}_{i}$ and $\hat{\mathbf{b}}^{t}_{i}$ represent the locations and their associated uncertainty of the best-predicted trajectory of agent $i$ at timestamp $t$. ${\bm{\mu}}^{t}_{i}$ is the locations of all predicted trajectories of agent $i$ at timestamp $t$. ${\rm CEL}$ is the cross-entropy loss.


\section{Hierarchical Lane Transformer}
% [You never explained this before, I think you should;
% huge is a subjective word. Replace it with great/important/significant;
% Remind that you have defined before that a lanelet is a group of lane segments, and explain therefore the intuition of using lanelets in a hierarchical way. The most important thing in a paper is to explain the intuition, if you just describe as you understand it it will be very hard for the reader to understand;
% As the other unselected ...;
% I though we multiplied after the softmax. I think multiplying before the softmax can have bad effects, as if the product qk is negative (and therefore should have low impact), and we multiply with a low alpha, it will have the adverse effect and reduce the penalty]
%By limiting the radius of the local regions, we reduce the computational complexity of Agent-Agent Transformer and Agent-Lane Transformer. However, 
The number of agent-lane edges in the local region is still very large, even if we limit the radius of the local regions. When the model performs the agent-lane interaction for every timestamp, it suffers from great time complexity and space complexity. In addition, not all lane segments in the range of the local regions have an impact on the agents' future behavior. Since a lanelet can be viewed as a set of lane segments, we can filter out the unuseful lanelets and lane segments belonging to them to reduce the computational complexity. Thus we propose the Hierarchical Lane Transformer and apply it in the agent-lane interaction module to only select lanelets that are most important to the target agent. As the other unselected lanelets would have scarcely any influence on the target agent, this does not decrease performance. We will demonstrate it in the ablation studies.\\

Specifically, the hierarchical lane transformer consists of an Agent-Lanelet Transformer and an Agent-Lane Transformer. The Agent-Lanelet Transformer has the same architecture as the Agent-Lane Transformer. We take the average position and the average position vector of all lane segments of lanelet $\Xi$ as the position $\mathbf{p}_{\Xi}$ and position vector $\mathbf{d}_{\Xi}$ of the lanelet $\Xi$. We create the edge embedding $\mathbf{z}_{i\Xi}$ between agent $i$ and lanelet $\Xi$ as follows:
\begin{align}
    &\mathbf{z}_{i\Xi} = \phi_{\rm{lanelet}}\Big([\mathbf{R}^{\top}_{i}(\mathbf{d}_{\Xi}),\mathbf{R}^{\top}_{i}(\mathbf{d}_{i\Xi}),\mathbf{d}_{i2\Xi}, l_{i\Xi},\mathbf{v}_{i2\Xi}, \mathbf{h}_{i2\Xi}, \mathbf{a}_{\Xi}] \Big)
\end{align}

In the first step, the Agent-Lanelet Transformer performs the scaled dot-product attention and yields a score $\bm{\alpha}^{t}_{i\Xi}$ for each lanelet to identify the most probably lanelets that can affect the target agent's motion.\\

In the second step, only lane segments that belong to the top-ranking lanelets are taken into account in calculating agent-lane interactions. To enhance the influence of the lanelet's score $\bm{\alpha}^{t}_{i\Xi}$, we multiply the scaled dot-product in Agent-Lane Transformer with $\bm{\alpha}^{t}_{i\Xi}$ before softmax function:
\begin{align}
    &\bm{\alpha}^{t}_{i\xi} = \bm{\alpha}^{t}_{i\Xi}\cdot {\rm softmax}\Big (\frac{{\mathbf{q}^{t}_i}^{\top}}{\sqrt{d_k}} \cdot \mathbf{k}^{t}_{i\xi}  \Big) 
\end{align}

where lane segment $\xi$ belongs to lanelet $\Xi$. The hierarchical lane transformer module not only reduces the computational complexity of agent-lane interaction module but also prevents the overfitting caused by complex road network in some cases (e.g. intersections).
% @
% The number of lane vectors is about 700-1000 in the local region within 50m radius, it’s to expensive to compute the AL interaction at each timestamp. 

% can make fast multi-agent motion prediction

%  can
% make fast multi-agent motion prediction

% #todo
% ) lanelet ranking: the score(alpha) is obtained by the agent-lanelet interaction module, the alpha of agent_lanelet 
% b) Lane ranking: The lanelet classification is obtained
% with a linear layer on the graph encoding, followed by a
% sigmoid activation. The ground-truth is defined by a 1 for
% all lanelets where the future car position is inside the lanelet
% polygon and 0 otherwise. The loss is a binary cross-entropy
% added to the pixel-wise loss of Eq. 2 with a 1e−2 coefficient.
% Since only a fraction of the lanelets will actually be useful to
% represent the future car location, we can compute the lanelevel rasters only for a subselection of lanelets, saving more
% computation. We use the classification score clane predicted
% by the network to select only the top k ranking lanelets, and
% only compute and project the lane raster for these. Since
% the raster predictions for the other unselected lanelets would
% have been very close to zero anyway, this does not decrease
% performance at all, as demonstrated in Sec.
% See~\autoref{tab:sample}, \autoref{fig:sample-drawing}, \autoref{fig:sample-plot}, \autoref{fig:sample-listing}.




==> chapters/METHOD2.tex <==

\chapter{Prediction_Framework}\label{chapter:Prediction_Framework}
In this chapter 

\subsection{Temporal Hierarchical Scene Graph Neural Networks}
For HiVT’s outstanding performance, we adopt its symmetrical representation method and its local-global mechanisms. Specifically, the traffic scene at each timestamp is divided into a set of local regions, each corresponds to one agent and centered at it. We employ a novel local encoder to extract agents’ spatial-temporal features from their associated local regions. The local encoder operates the temporal scene graph in two stages. In the first stage, it models the agent-agent interactions and agent-lane interactions per time step and use a temporal module to capture the temporal dependecies across traffic scenes. In the second stage, it use the updated agents' features to update the ralative spatial relationships between entities and models the agent-agent interaction per time step again, followed by a temporal module with classification token and a agent-lane module with larger perspective field, we obtain the final updated features for each agent.

\subsubsection{Agent-Agent Transformer (first stage)}

\begin{align}
    &\mathbf{q}^{t}_i = \mathbf{W}^{Q^{space}}\mathbf{z}^{t}_i\\
    &\mathbf{k}^{t}_{ij} = \mathbf{W}^{K^{space}}\mathbf{z}^{t}_{ij}\\
    &\mathbf{v}^{t}_{ij} = \mathbf{W}^{V^{space}}\mathbf{z}^{t}_{ij}
\end{align}

\begin{align}
    &\bm{\alpha}^{t}_i = \mathbf{W}^{Q^{space}}\mathbf{z}^{t}_i\\
    &\mathbf{k}^{t}_{ij} = \mathbf{W}^{K^{space}}\mathbf{z}^{t}_{ij}\\
    &\mathbf{v}^{t}_{ij} = \mathbf{W}^{V^{space}}\mathbf{z}^{t}_{ij}
\end{align}

\begin{align}
    % &\bm{\alpha}^{t}_i = softmax(\frac{\mathbf{q}^{t}_i}{\sqrt{d_k}}[\{\mathbf{k}^{t}_{ij}\}_{j\in \mathcal N_{i}}]) 
    % &\bm{\alpha}^{t}_i =  \rm{softmax}\Bigg (\frac{{\mathbf{q}^{t}_i}^{\top}}{\sqrt{d_k}} \cdot \Big [\{\mathbf{k}^{t}_{ij}\}_{j\in \mathcal N_{i}}\Big ] \Bigg) \\
    &\bm{\alpha}^{t}_{ij} =  \rm{softmax}\Bigg (\frac{{\mathbf{q}^{t}_i}^{\top}}{\sqrt{d_k}} \cdot \mathbf{k}^{t}_{ij}\Bigg) \\
    &\mathbf{m}^{t}_{i} = \sum_{j\in \mathcal N_{i}}\bm{\alpha}^{t}_{ij}\mathbf{v}^{t}_{ij}\\
    &\mathbf{g}^{t}_{i} =  \rm{sigmoid}(\mathbf{W}^{ \rm{gate}}[\mathbf{z}^{t}_{i},\mathbf{m}^{t}_{i}])\\
    &\hat{\mathbf{z}}^{t}_{i} = \mathbf{g}^{t}_{i}\odot\mathbf{W}^{ \rm{self}}\mathbf{z}^{t}_{i}+(1-\mathbf{g}^{t}_{i})\odot\mathbf{m}^{t}_{i}
\end{align}




\begin{align}
   &\mathbf{Q}_{i} = \mathbf{S}_{i}\mathbf{W}^{Q^{time}}\\
   &\mathbf{K}_{i} = \mathbf{S}_{i}\mathbf{W}^{K^{time}}\\
   &\mathbf{V}_{i} = \mathbf{S}_{i}\mathbf{W}^{V^{time}}\\
   &\hat{\mathbf{S}}_{i} = \rm{softmax}\Bigg (\frac{{\mathbf{Q}_i}{\mathbf{K}^{\top}_i}}{\sqrt{d_k}} + \mathbf{M}\Bigg)\mathbf{V}_{i} \\
\end{align}

\begin{equation*}
\mathbf{M}_{uv} = \begin{cases}
 -\infty &\text{if u<v}\\
0 &\text{otherwise}\\
\end{cases}
\end{equation*}

% \begin{equation}
% \begin{aligned}
% ;
% \end{aligned}           
% \end{equation}
% @
Every agent has its own pattern, they move with different trajectories and have different goals. They adjust their trajectories by implicitly inferring about the behavior of surrounding agents. These surrounding agents in-turn are also influenced by their immediate neighborings and could alter their behaviour over time. 

To accurately predict the future behavior of agents in the traffic scene, we need a model to learn and understand the interaction between agents. We use a multi-head cross-attention block to learn the interaction relationships and the importance of the influence of different surrounding agents on the center agent for each local region at each time step.


Speciafically, firstly, we rotate all translation-invariant but not rotation-invariant local vectors according to the heading $\theta^{T}_{i}$ of central agent $i$ at the current timestamp $T$ and apply Multi-Layer Perceptrons(MLPs) on its node attributes and edge attributes, then we 
obtain the central agent $i$'s temporal node embedding $\mathbf{z}^t_i$ and any of its associated temporal edge embedding $\mathbf{z}^t_{ij}$ which is conected with neighboring agent $j$: 
\begin{align}
    &\mathbf{z}^{t}_{i} = \phi_{\rm{center}}\Big([\mathbf{R}^{T}_{i}\mathbf{d}^{t}_i, \mathbf{R}^{T}_{i}\mathbf{v}^{t}_i, \mathbf{R}^{T}_{i}\mathbf{h}^{t}_i, s^{t}_i, \Delta t^{t}, \mathbf{a}_{i}] \Big)\\
    &\mathbf{z}^{t}_{ij} = \phi_{\rm{nbr}}\Big([\mathbf{R}^{T}_{i}\mathbf{d}^{t}_{j}, \mathbf{R}^{T}_{i}\mathbf{d}^{t}_{ij}, \mathbf{R}^{T}_{i}\mathbf{v}^{t}_{ij}, l_{ij}, s_{ij}, \mathbf{d}^{t}_{j2i}, \mathbf{v}^{t}_{j2i}, \mathbf{h}^{t}_{j2i}, \mathbf{a}_{j}] \Big)
    %\mathbf{p}^{t}_{j}-\mathbf{p}^{t-1}_{j}
    %&\mathbf{e_a} = \{\mathbf{d}^{t}_{ij}, \mathbf{v}^{t}_{ij}, l_{ij}, s_{ij},\mathbf{d}^{t}_{j2i},\mathbf{v}^{t}_{j2i},\mathbf{a}^{t}_{j2i}|t=0,...,19;i,j=1,...,N\}\\  
\end{align}
where $\phi_{\rm{center}}$ and $\phi_{\rm{nbr}}$ are MLP blocks and $\mathbf{R}^{T}_{i}$ is the rotation matrix parameterized by the heading $\theta^{T}_{i}$.
After rotation transformation, both node and edge attributes are translation and rotation invaraiant, their embeddings also inherits these properties. We then encode the central agent $i$'s node embedding $\mathbf{z}^t_i$ and its associated edge embedding $\mathbf{z}^t_{ij}$ by learnable matrices to obtain the query, key and value vectors:
 \begin{align}
    &\mathbf{q}^{t}_i = \mathbf{W}^{Q^{space}}\mathbf{z}^{t}_i\\
    &\mathbf{k}^{t}_{ij} = \mathbf{W}^{K^{space}}\mathbf{z}^{t}_{ij}\\
    &\mathbf{v}^{t}_{ij} = \mathbf{W}^{V^{space}}\mathbf{z}^{t}_{ij}
\end{align}
where $\mathbf{W}^{Q^{space}}$, $\mathbf{W}^{K^{space}}$ and $\mathbf{W}^{V^{space}}$ are the query, key and value matrix for linear transformation. The cross attention block receives query $\mathbf{q}^{t}_i$, key $\mathbf{k}^{t}_{ij}$ and value $\mathbf{v}^{t}_{ij}$ as inputs, and performs the scaled  dot-product attention with a gating function $\mathbf{g}^{t}_{i}$ [] as:
% where $\mathbf{W}^{Q^{space}}$, $\mathbf{W}^{K^{space}} and $\mathbf{W}^{V^{space}} are the learnable matrices  query, key and value vectors respectively. (查看attention 说明，sca;ed.dot production attention)
%\begin{align}
%     &\bm{\alpha}^{t}_i = \mathbf{W}^{Q^{space}}\mathbf{z}^{t}_i\\
%     &\mathbf{k}^{t}_{ij} = \mathbf{W}^{K^{space}}\mathbf{z}^{t}_{ij}\\
%     &\mathbf{v}^{t}_{ij} = \mathbf{W}^{V^{space}}\mathbf{z}^{t}_{ij}
% \end{align}
\begin{align}{} \label{attention}
    % &\bm{\alpha}^{t}_i = softmax(\frac{\mathbf{q}^{t}_i}{\sqrt{d_k}}[\{\mathbf{k}^{t}_{ij}\}_{j\in \mathcal N_{i}}]) 
    &\bm{\alpha}^{t}_i =  \rm{softmax}\Bigg (\frac{{\mathbf{q}^{t}_i}^{\top}}{\sqrt{d_k}} \cdot \Big [\{\mathbf{k}^{t}_{ij}\}_{j\in \mathcal N_{i}}\Big ] \Bigg) \\

    &\mathbf{m}^{t}_{i} = \sum_{j\in \mathcal N_{i}}\bm{\alpha}^{t}_{ij}\mathbf{v}^{t}_{ij}\\
    &\mathbf{g}^{t}_{i} =  \rm{sigmoid}(\mathbf{W}^{ \rm{gate}}[\mathbf{z}^{t}_{i},\mathbf{m}^{t}_{i}])\\
    &\hat{\mathbf{z}}^{t}_{i} = \mathbf{g}^{t}_{i}\odot\mathbf{W}^{ \rm{self}}\mathbf{z}^{t}_{i}+(1-\mathbf{g}^{t}_{i})\odot\mathbf{m}^{t}_{i}
\end{align}
where $d_k$ is the dimensionality of the query and key and $\mathcal N_{i}$ represents the surrounding agents of agent $i$. We further apply a MLP block and residual connections[] to obtain the first updated node embedding $\mathbf{s}^{t}_{i}$ of agent $i$ at timestamp $t$ which incorperates interactions between agents.


@
Spatio-temporal
graphs have nodes that represent the problem components
and edges that capture spatio-temporal interactions between
the nodes. 


@
The spatial edgeRNNs model the dynamics of
human-human interactions in the crowd and the temporal
edgeRNNs model the dynamics of individual motion of
each human in the crowd. 

@
####Prediction of future motion of surrounding vehicles is a
challenging problem due to the high number of latent variables involved, such as, the end goals of all drivers in the
scene and variability in driving style across different drivers.
Vehicle trajectories tend to be highly non-linear over longer
time horizons due to decisions made by the driver. Additionally, driver behavior tends to be inherently multi-modal,
where a driver could make one of many decisions under the

same traffic circumstances. Finally, interaction between vehicles tends to affect their motion. The large number of
possible configurations of all vehicles in a scene can make
this difficult to model

@
#####Following the success of transformer (transformer)  #interaction aware models. 
(Interaction aware models for
motion prediction take into account the effect of intervehicle interaction on the motion of vehicles.)

\subsubsection{Agent-Lane Transformer}
@
The road network plays a crucial role in motion predictions. Every agent has its implicit goal, we can't know their intentions ahead of time. However, the surrounding road network can indicate the future driving trajectories of the agents to a certain degree. To capture these implicit interactions between agents' trajectories and lane segments, we employ another multi-head cross-attention block. Similar as the agent-agent (Transformer) interaction module. According to the heading $\theta_i$ of central agent $i$,  we rotate the local lane segments, and their associated rotation-variant temporal edge attributes which are connected with the centeral agent i and encode them by a MLP block $\phi_{\rm{lane}}$ to obtain the edge embedding between agent $i$ and lane $\xi$:
\begin{align}
    &\mathbf{z}_{i\xi} = \phi_{\rm{lane}}\Big([\mathbf{R}^{T}_{i}(\mathbf{d}_{\xi}),\mathbf{R}^{T}_{i}(\mathbf{d}_{i\xi}),\mathbf{d}_{i2\xi}, l_{i\xi},\mathbf{v}_{i2\xi}, \mathbf{h}_{i2\xi}, \mathbf{a}_{\xi}] \Big)
\end{align}

%where $\phi_{\rm{lane}}$ is a MLP block and $\mathbf{a}_{\xi}$ is the semantic attributes of lane segment $\xi$. 

%\mathbf{p}^{1}_{\xi}-\mathbf{p}^{0}_{\xi}
%\mathbf{p}^{0}_{\xi}-\mathbf{p}^{T}_{i}
%&\mathbf{e_l} = \{\mathbf{d}_{i\xi}, \mathbf{d}_{i2\xi},l_{i\xi},\mathbf{v}_{i2\xi},\mathbf{a}_{i2\xi}|i=1,...,N;\xi==1,...,M\}\\


#equ:...
The another multi-head cross-attention block takes agent $i$'s node embedding $\mathbf{s}^{t}_{i}$ as query, the edge embedding $\mathbf{z}_{i\xi}$ between central agent $i$ and lane segment $\xi$ as key and value, and performs the scaled dot-product attention the same as the agent-agent interaction module.

By moduling the agent-agent and agent-lane interaction, we obtain the spatial node embedding $\mathbf{s}^{t}_{i}$ of agent $i$ at timestamp $t$. %which incorperates interactions between agents and between agents and lanes.

@todo, 变量名

in practice we set the radius $d = 20$



\subsubsection{Hierarchical Agent-Lane Transformer}
:...


\subsubsection{Temporal Transformer}

future motions of traffic agents in highly
dynamic

We get the encoded scene at each timestamp
Since motion prediction can be viewed as a sequence classification
or sequence generation task, a
@
#
However, most previous approaches ... don't take the map influence at each timestamp into account, pattern in the past affect the pattern in the future.
apply a fully connected layer to the social tensor. 

unlike the most approaches which only encode the temporal historical trajectory a single agent or agents in a local region, we consider the temporal historical traffic scenes include agents' dynamic and surrounding lane segments at each timestamp. 

As a remedy, we propose to consider the whole scene at any timestamp 
can be expected to help learn locally useful features within
the 
both of which help address the problem described above.

@Inferring the future motions of traffic agents relies heavily on the historical information. we encode the whole temporal scene graph. 

@The historical information plays a crucial role in inferring the traffic agents' dynamics in the future. We treat the encoded traffic scene at each timestamp as an entirety and use a temporal transformer to capture temporal dependencies of all historical traffic scenes. Specifically, we add the learnable positional embeddings[] to the agent $i$'s spatial node embedding ${\mathbf{s}^{t}_{i}}^{T}_{t=1}$ at each timestamp with, stack them into a matrix $\mathbf{S}_{i}$ and perform multi-head self-attentiondot as:
\begin{align}
   &\mathbf{Q}_{i} = \mathbf{S}_{i}\mathbf{W}^{Q^{time}}\\
   &\mathbf{K}_{i} = \mathbf{S}_{i}\mathbf{W}^{K^{time}}\\
   &\mathbf{V}_{i} = \mathbf{S}_{i}\mathbf{W}^{V^{time}}\\
   &\hat{\mathbf{S}}_{i} = \rm{softmax}\Bigg (\frac{{\mathbf{Q}_i}{\mathbf{K}^{\top}_i}}{\sqrt{d_k}} + \mathbf{M}\Bigg)\mathbf{V}_{i}\\
   &\mathbf{M}_{uv} = \begin{cases}
                     -\infty &\text{if u<v}\\
                    0 &\text{otherwise}\\
                    \end{cases}
\end{align}

where $\mathbf{W}^{Q^{time}}$, $\mathbf{W}^{K^{time}}$ and $\mathbf{W}^{V^{time}}$ are the query, key and value matrix for linear transformation.
$\hat{\mathbf{S}}_{i}$ summarize the spatial-temporal features of agent $i$ at each timestamp.

 %By sequentially modeling agent-agent interactions, agent-lane interactions and temporal dependencies (transformer), we obtain the spatial-temporal node embedding $\mathbf{s}^{t}_{i}$ of agent $i$. %which incorperates interactions between agents and between agents and lanes.


(... (Unlike other methods,)
Specifically, firstly, similar to BERT, ..
we extand the embeddings with an extra learnable token 
sT +1 ∈ Rdh to the end of the input sequence. This token is used as the aggregate sequence representation for classification
tasks. (classify different manuevers of agents)

#equ..  +learnable token, positonal embeddings.. ()
%%#看BERT怎么写
its input representation of temporal transformer $S$ is
constructed by summing the embeddings(), and positional embeddings.
To obtain temporal dependent scene features, we compute the self attention of $S$:


@
expect the hidden states of an LSTM
to capture these time varying motion-properties.

#
Agent history encoding. The agent history encoding is obtained by concatenating the output of three sources:

3. MCG blocks applied to the set of history elements. Each element in the set consists of a historical position and


where the second argument is the input context vector to MCG, which in this case is a concatenation of the modeled
agent’s history embedding, and the AV’s interaction embedding

@is the temporal mask that
enforces the tokens only attend to the preceding time steps.
We don't (@看Scene transformer 怎么写)

Citation test~\parencite{latex}. and  \parencite{ngiam2021scene}
\begin{figure}[htbp]
\centering
%\subfigure[]{
\includegraphics[width=14cm]{images/framework1.pdf}
\caption{Overall Framework\cite{zhou2022hivt}}
\label{Overall Framework}
\end{figure}

\begin{figure}[htbp]
\centering
%\subfigure[]{
\includegraphics[width=14cm]{images/le.pdf}
\caption{Local Encoder}
\label{Local_Encoder}
\end{figure}

\subsubsection{Second Part}
\label{sec:Second Part}
We set a larger radius of local regions in this stage to have a larger perceptual field of surrounding environment. In practice we set the radius $d = 50$. 
After sequentially modeling agent-agent interactions, agent-lane interactions and temporal transformer, we obtain spatial-temporal scene features of local regions, all agents' node embeddings are updated, we then update the edge embeddings between agents as %and between agents and lanes as following:
\begin{align}
    %&\mathbf{z}^{t}_{i} = \phi_{\rm{center}}\Big([\mathbf{R}^{T}_{i}\mathbf{d}^{t}_i, \mathbf{R}^{T}_{i}\mathbf{v}^{t}_i, \mathbf{R}^{T}_{i}\mathbf{h}^{t}_i, s^{t}_i, \Delta t^{t}, \mathbf{a}_{i}] \Big)\\
    &\mathbf{z}^{t}_{{ij}_{2}} = \phi_{\rm{nbr}_2}\Big([\mathbf{s}^{t}_{i},\mathbf{z}^{t}_{ij}] \Big)
    %&\mathbf{z}_{{i\xi}_{2}} = \phi_{\rm{lane}_2}\Big([\mathbf{s}^{t}_{i},\mathbf{z}_{{i\xi}] \Big)
\end{align}

#equ: aa, al

We use the updated agents’ nodes and edges embeddings between agents to model another same agent-agent interaction module and obtain new node embedding $\mathbf{s}^{t}_{i}$. In the first A-A interaction module, the agents lack the information about the road network, which could affect their behaviors and interactions. Thus, we apply it again, after all agents are incorporated with the road network information. 

We then model another same temporal transformer with an extra learnable classification token similar as BERT[] and a temporal mask $\mathbf{M}$ that
enforces the tokens only attend to the preceding time steps:
\begin{align}
    &\hat{\mathbf{S}}_{i} = \rm{softmax}\Bigg (\frac{{\mathbf{Q}_i}{\mathbf{K}^{\top}_i}}{\sqrt{d_k}} + \mathbf{M}\Bigg)\mathbf{V}_{i}\\
    &\mathbf{M}_{uv} = \begin{cases}
                     -\infty &\text{if u<v}\\
                    0 &\text{otherwise}\\
                    \end{cases}
\end{align}

We update the edge embeddings between agents and lanes as: 
\begin{align}
    &\mathbf{z}_{{i\xi}_{2}} = \phi_{\rm{lane}_2}\Big([\mathbf{s}^{t}_{i},\mathbf{z}_{i\xi}]\Big)
\end{align}

We input the updated extra classification token as query and updated edge embeddings $\mathbf{z}_{{i\xi}_{2}}$ between agent $i$ and lane $\xi$ as key and value to another same agent-lane interaction module. We obtain the final node embedding $\mathbf{h}_{i}$ of the central agent $i$. $\mathbf{h}}_{i}$
summarizes the fused rich spatial-temporal features of the agent $i$'s surrounding environment and incoperates the iterative interatations between agents and between agents and lanes.

\subsection{Global}
\subsubsection{Global Interaction Module}

The local encoder output represents the features of the central agent within its local region, but it does not incorporate the pairwise interactions between local regions and lack the longr-ange dependencies in the scene. To address these issues, we introduce a global interaction module similar as HiVT[] for high-order interactions.

(to bridge inter-frame geometric relationships when performing message passing among local regions.) 

Similar as the agent-agent interaction module, we use a MLP $\phi_{rel}$ to obtain the edge embedding $e_{ij}$ between agent $i$'s and agent $j$'s local regions:

\begin{align}
    &\mathbf{z}_{ij} = \phi_{\rm{rel}}\Big([\mathbf{R}^{T}_{i}\mathbf{d}^{t}_{ij}, \mathbf{R}^{T}_{i}\mathbf{v}^{t}_{ij}, l_{ij}, s_{ij}, \mathbf{d}^{t}_{j2i}, \mathbf{v}^{t}_{j2i}, \mathbf{h}^{t}_{j2i}] \Big)
\end{align}

We take the local node embedding $\mathbf{h}_i$ as query, the concatenation of $\mathbf{h}_j$ and $&\mathbf{z}_{ij}$ as key and value:
\begin{align}
    & \widetilde{\mathbf{q}}_i = \mathbf{W}^{Q^{global}}\mathbf{h}_i\\
    & \widetilde{\mathbf{k}}_{ij} = \mathbf{W}^{K^{global}}[\mathbf{h}_j,\mathbf{e}_{ij}]\\
    & \widetilde{\mathbf{v}}_{ij} = \mathbf{W}^{V^{global}}[\mathbf{h}_j,\mathbf{e}_{ij}]
\end{align}

where $\mathbf{W}^{Q^{global}}$, $\mathbf{W}^{K^{global}}$ and $\mathbf{W}^{V^{global}}$ are query, key and value matrix for linear transformation. A same multi-head cross-attention block takes them as input and outputs agent $i$'s new updated node embedding $\widetilde{\mathbf{h}}_i$. To address this issue, we introduce a mixture density network to output 

\subsection{Multimodal Future Decoder}

In a complex traffic scene, based solely on past observations of the target agent and its surrounding environment, we cannot accurately predict its future maneuver. For example, an agent at the intersection could go straight, turn left, turn right, etc. 

To address this issue, we apply a mixture density network[] with gru[] as decoder to output multimodal trajectories for each agent. The decoder receives 

Specifically, we tile all agents' global representations $\widetilde{\mathbf{h}}$ with shape $[F, N, D]$ and local representations $\mathbf{h}$ with shape $[N, D]$ $H$ and $F$ time, where $F$ is the number of mixture components, $N$ is the number of agents, $D$ is the number of agents' features and $H$ is the number of future steps. The gru receives the tiled global representations with shape $[H, F \times N, D]$ as inputs and the tiled local representations with shape $[1, F \times N, D]$ as the initial hidden state. We further apply two different MLP blocks $\phi_{\rm{loc}}$, $\phi_{\rm{unc}}$ which take the outputs of gru $\mathbf{o}$ as inputs and output locations $\bm{\mu}$ with shape $[F, N, H, 2]$ and the associated uncertainty $\mathbf{b}$ with shape $[F, N, H, 2]$. We apply another MLP block $\phi_{\rm{prob}}$ with the concatenation of $\mathbf{h}$ and $\widetilde{\mathbf{h}}$ as inputs to obtain the probability $\bm{\pi}$ of possible future trajectories of all agents:

\begin{align}
    &\mathbf{o} = \rm{GRU}([\widetilde{\mathbf{h}}, \mathbf{h}])\\
    &\bm{\mu} = \phi_{\rm{loc}}(\mathbf{o})\\
    &\mathbf{b} = \phi_{\rm{unc}}(\mathbf{o})\\
    &\bm{\pi} = \phi_{\rm{prob}}([\widetilde{\mathbf{h}}, \mathbf{h}])
\end{align}

 and output the 

µt i;f 2 R2 and
its associated uncertainty bt i;f 2 R2 of the agent per future time step in the local coordinate frame. 

a mixture model is a probabilistic model for representing the presence of . Formally a mixture model corresponds to the mixture distribution that represents the probability distribution of observations in the overall population. 

#todo Each traffic agent can have F distinct futures, their motions are inherently multimodal.

The future motions of traffic agents are inherently multimodal. Thus, we parameterize the distribution of future trajectories as a mixture model where each mixture component is a Laplace distribution. The predictions are made for all
agents in a single shot.

@
For each agent $i$ and each component $f$, we tile its global and local representations $F$ and $N$ time respectively. 


The gru receives the tiled global representations with shape [H, F x N, D] as inputs and the tiled local representations with shape [1, F x N, D] as the initial hidden state and output the location µt i;

a GRU[] receives the local and the global representations as inputs and the initial hidden state and outputs the location µt i;f 2 R2 and
its associated uncertainty bt i;f 2 R2 of the agent per future time step in the local coordinate frame. Specifically, we expand the which have the shape of [H, F x N, D]. repeat the local representations which have the shape of [1, F x N, D]

The output tensor of the regression head has the shape of [F; N; H; 4], where F is the number of mixture components, N is the number of
agents in the scene, and H is the number of predicted future
time steps. We also use another MLP followed by a softmax
function to produce the mixing coefficients of the mixture
model for each agent, which have the shape of [N; F].

In order to allow the decoder to output F distinct futures, we perform
the following operations. The decoder receives as input a tensor of shape [A; T; D] corresponding to
A agents across T time steps and D feature dimensions. The following series of simple operations
restructures the representation to predict F futures. First, the representation is tiled F times to
generate [F; A; T; D]. For computational
simplicity, the resulting representation is propagated through a small MLP to produce a return a
tensor of the shape [F; A; T; D].

\subsection{Loss Function}

According to our observation, the tracking data of Argoverse dataset $1$ is noisy. Compared to Gaussian negative log-likelihood loss, Laplace negative log-likelihood loss is more robust to outliers, thus we design the decoder Sec. in this way so that it predicts a parameterization of the
location and its associated uncertainty corresponding to a Laplace distribution[] (Meyer & Thakurdesai, 2020). We use the winner-take-all strategy. We only  
apply the loss to the best-predicted trajectory which is defined as the one that has the minimum endpoint error. Our final loss consists of the regression loss $\mathcal{L}_{\rm{reg}}$ and the classification loss $\mathcal{L}_{\rm{cls}}$:
\begin{align}
    &\mathcal{L}_{reg} = -\frac{1}{NH}\sum^N_{i=1}\sum^{T+H}_{t=T+1}\log P\Big(\mathbf{R}^{T}_{i}(\mathbf{p}^{t}_{i}-\mathbf{p}^{T}_{i}) | \hat{\bm{\mu}}^{t}_{i},\hat{\mathbf{b}}^{t}_{i}\Big)\\
    &\overline{\bm{\pi}}_{i}={\rm softmax}\Big(-\sum^{T+H}_{t=T+1}\lVert \hat{\bm{\mu}}^{t}_{i},\mathbf{R}^{T}_{i}(\mathbf{p}^{t}_{i}-\mathbf{p}^{T}_{i}) \lVert \Big) \\
    &\mathcal{L}_{cls} = {\sum^N_{i=1}}{\rm CEL}(\overline{\bm{\pi}}_{i}, \hat{\bm{\pi}}_{i})\\
    &\mathcal{L}=\mathcal{L}_{\rm{reg}} + \mathcal{L}_{\rm{cls}}
\end{align}
% We parameterize the distribution of agent's future trajectory as a Laplace distribution. 

The loss function $\mathcal{L}$ consists of the regression loss $\mathcal{L}_{\rm{reg}}$ and $\mathcal{L}_{\rm{cls}}$. $\hat{\bm{\mu}}^{t}_{i}$ and $\hat{\mathbf{b}}^{t}_{i}$ represent the predicted location and its associated uncertainty of the best-predicted trajectory of agent $i$ at timestamp $t$. ${\rm CEL}$ is the cross-entropy loss.


\subsection{Hierarchical Lane Transformer}

By limiting the radius of the local regions, we reduce the computational complexity of agent-agent and agent-lane interaction module. However the number of agent-lane edges in local region with radius $d=20$ is still very large. 

When the model performs the agent-lane interaction for every timestamp, it suffers from huge time complexity and huge space complexity. In addition, not all lane segments in the range of the local regions have an impact on the agents' future behavior. Thus we propose the hierarchical lane transformer and apply it in the agent-lane interaction module to only select lanelets that are most important to the target agent. The other unselected lanelets would
have scarcely any influence on the target agent, this does not decrease performance, as demonstrated in Sec.

Specifically, the hierarchical lane transformer consists of agent-lanelet-interaction and agent-lane-interaction modules. The agent-lanelet interaction module has the same architecture as the agent-lane-interaction module. We take the average position and the average position vector of all lane segments of lanelet $\Xi$ as the position $\mathbf{p}_{\Xi}$ and position vector $\mathbf{d}_{\Xi}$ of lanelet $\Xi$. We create the edge embedding $\mathbf{z}_{i\Xi}$ between agent $i$ and lanelet $\Xi$ as following:
\begin{align}
    &\mathbf{z}_{i\Xi} = \phi_{\rm{lanelet}}\Big([\mathbf{R}^{T}_{i}(\mathbf{d}_{\Xi}),\mathbf{R}^{T}_{i}(\mathbf{d}_{i\Xi}),\mathbf{d}_{i2\Xi}, l_{i\Xi},\mathbf{v}_{i2\Xi}, \mathbf{h}_{i2\Xi}, \mathbf{a}_{\Xi}] \Big)
\end{align}

In the first step, the agent-lanelet interaction module performs the scaled dot-product attention and yields a score $\bm{\alpha}^{t}_{i\Xi}$ for each lanelet to identify most probably lanelets that can affect the target agent's motion. 

In the second step, only lane segments that belong to the top ranking lanelets are taken into account in calculating agent-lane interactions. In order to enhance the influence of lanelet's score $\bm{\alpha}^{t}_{i\Xi}$, we multipy the scaled dot-product in agent-lane interaction module with $\bm{\alpha}^{t}_{i\Xi}$ before softmax function:
\begin{align}
    &\bm{\alpha}^{t}_{i\xi} = {\rm softmax}\Big (\frac{{\mathbf{q}^{t}_i}^{\top}}{\sqrt{d_k}} \cdot \mathbf{k}^{t}_{i\xi} \cdot \bm{\alpha}^{t}_{i\Xi} \Big) 
\end{align}

where lane segment $\xi$ belongs to lanelet $\Xi$. The hierarchical lane transformer module not only reduces the computational complexity of agent-lane
interaction module but also prevents overfitting caused by complex road network in some cases (e.g. intersections) , as demonstrated in Sec.
@
The number of lane vectors is about 700-1000 in the local region within 50m radius, it’s to expensive to compute the AL interaction at each timestamp. 

can make fast multi-agent motion prediction

 can
make fast multi-agent motion prediction

#todo
) lanelet ranking: the score(alpha) is obtained by the agent-lanelet interaction module, the alpha of agent_lanelet 
b) Lane ranking: The lanelet classification is obtained
with a linear layer on the graph encoding, followed by a
sigmoid activation. The ground-truth is defined by a 1 for
all lanelets where the future car position is inside the lanelet
polygon and 0 otherwise. The loss is a binary cross-entropy
added to the pixel-wise loss of Eq. 2 with a 1e−2 coefficient.
Since only a fraction of the lanelets will actually be useful to
represent the future car location, we can compute the lanelevel rasters only for a subselection of lanelets, saving more
computation. We use the classification score clane predicted
by the network to select only the top k ranking lanelets, and
only compute and project the lane raster for these. Since
the raster predictions for the other unselected lanelets would
have been very close to zero anyway, this does not decrease
performance at all, as demonstrated in Sec.
See~\autoref{tab:sample}, \autoref{fig:sample-drawing}, \autoref{fig:sample-plot}, \autoref{fig:sample-listing}.


==> pages/abstract.tex <==
\chapter{\abstractname}
% @
Predicting the future motions of the nearby agents is essential for an autonomous vehicle to take safe and effective actions. In this paper, we propose THSGN, a framework using Temporal Hierarchical Scene Graph Neural Networks (THSGN) with Projected vectorized representations for tackling multi-agent trajectory prediction. Projected vectorized representation models the temporal traffic scene as a temporal graph which is constructed by a set of vectors. These vectors represent the entities, i.g., agents, road network, and their spatial relative relationships. All relative spatial features between these entities under this representation are both translation- and rotation-invariant. Based on this scene representation, THSGN deeply captures the spatial-temporal features across agents, road network, interactions among them, and temporal dependencies of the temporal traffic scene. This prediction framework can predict multimodal future trajectories for all agents simultaneously, plausibly, and accurately. Meanwhile, we propose a hierarchical lane transformer for capturing the interactions between agents and road network, which filters the surrounding road network and only keeps the most probable lane segments where the target agent could move to in the future time horizon. Without sacrificing the prediction performance, this greatly reduces the computational burden. Experiments show that THSGN achieves state-of-the-art performance on the Argoverse motion forecasting benchmark. %lane segments(HD-map)

%In this paper, we propose THSGN with projected vectorized representation, Either explain the full acronym or just use he abreviation: 



% . All entities are represented as sets of vectors.


% a set of vectors . finely describes the relative spatial relationships between
% entities in the traffic scene

 
% Our approach can finely describe the relative spatial relationship , 

% our method
% can effectively and efficiently model a large number of
% agents in the scene. 



% the agent could move to in the future time horizon. 
% todo
% THSGN reaches 1nd 
% We apply our method to the Argoverse Motion
% Forecasting Benchmark and achieve 1st place on the online
% leaderboard.
% Predicting the motion of multiple agents is an essential step in the pipeline of the autonomous driving. It helps autonomous driving vehicles to plan their future actions and prevent potential accidents. However, the traffic scene is highly complex. It contains agents'trajectories, HD-map, spatial relationships and interactions among them. The prediction model needs to take these entities as inputs and outputs plausible multimodal trajectories that the target agents could take in the future. An example of multi-agent trajectory prediction is shown in \ref{trajectory prediction_vector}.


% \begin{figure}[htbp]
% \centering
% %\subfigure[]{
% \includegraphics[width=12cm]{bilds/tp.png}
% \caption[trajectory prediction]{[]}
% \label{An example of multi-agent trajectory prediction. The blue and the orange trajectory present two distinct predictions and the scores indicate likelihood of the corresponding trajectory.[st]  }
% \end{figure}

% %In this work, we propose THSGNNs, a novel framework for predicting multi-agent trajectory simultaneously. Our model architecture employs 

% %attention to combine spatial and temporal features of the sequential traffic scene graphs.
% % lane segments within a certain range of the target agent,

% The traditional models usually use Kalman filters[] and it extentions[][] in conjunction with rule-based methods to predict multiple possible future trajectories. Recently, learning-based approaches are widely used, for its benefits of modeling agents' multimodal behaviors.  CNNs-based models[][][] renders the traffic scene into a rasterized bird’s eye view image with multi-channels and use convolutional neural networks to capture hidden features of the traffic scene. However these models are limited to a restricted image size and CNNs have limited receptive fields. To tackle these issues, vectorized approaches are proposed. VectorNet-based models [1]–[4], LaneGCN-based models[][][], and TPCN-based models[][] represent the road network and agents' trajectories of the traffic scene by a set of vectors or point clouds. They use graph neural networks[][][gat], attention mechasims[][], transformer or PointNet[][][] to encode the constructed graph or point clounds. However, the traffic scene is viewed different from the perspective of different agents. Most of these approaches select one target agent each time and take it as the central reference to perform coordinate transformation on the entire scene, which is not symmetric for the other agents and results in only one prediction at a time. It is inefficient and not robust to the coordinate transformation. To alleviate these problems, HiVT[] takes a summetric way to encode the traffic scene. It divides the traffic scene into a set of local regions, each corresponds to one agent and centered at it. It uses a local encoder to extract agents'features from their associated local regions and a global encoder to capture long range dependencies and interactions among local regions. 

% %   Besides, . Most 
% % and other agents.  results i
% % -----those methods have to forward multiple
% % times with each agent as the reference agent.% these approaches neglect the symmetries of the


% % To avoid 

% %  when a large number of 
% % agents in the scene need to be predicted@

% % as a temporal graph in which node features and edge features are updated at each timestamp. 

% % most approaches
% % aforementioned select a fixed agent as the global reference in the
% % coordinate system, which 

% For HiVT's outstanding performance, we adopt its symmetrical representation method and its local-global mechanisms and propose an optimized prediction framework: THSGN with projected vectorized representation. Projected vectorized representation treats the temporal traffic scene as a temporal graph in which nodes represent agents and edges represent relative spatial representations beween agents or between agents and lanes. Both nodes' and edges' features are updated at each timestamp. It encodes the traffic scene according to each target agent's view in one go. All relative spatial features between entities under this representation is both translation- and rotation-invariant. Projected vectorized representation not only avoids cumbersome coordinate transformations but also describes the relative spatial relationships in a more detail way. THSGN consists of diverse interaction modules and temporal dependencies modules. These modules are constructed based on the transformer structure. THSGN treats the traffic scene as an entirety and encodes the agents’ dynamics, surrounding lane segments and interactions among them across time steps. After updating nodes and edges embedding per timestamp, it   It deeply combines features across agents, HD-map, interactions among them and temporal dependencies of the temporal traffic scene. In addition, we present a hierarchical lane transformer module inside THSGN to capture the influence of the HD-map on the future motion of target agents. Unlike most approaches that use the full structural information of the surrounding HD map, the hierarchical lane transformer only selects the most probable lane segments where the agent could move to in the future time horizon. It greatly reduces the computation burden and enables the model to do faster predictions without sacrificing the prediction performance.

% Our contributions are summarized as follow:

% 1. We propose a novel scene representation method, namely projected vectorized representation. It not only finely describes the relative spatial relationships between entities in the traffic scene, but also guarantees the translation invariance and rotation invariance.

% 2. We propose a hierarchical lane transformer for capturing the interactions between agents and lane segments. It only selects lane segments that affects target agents the most for modelling the interactions, enabling much faster and equal accurate predictions and prevent overfitting to a certain degree.

% 3. Our designed novel model THSGN can make plausible and accurate predictions. THSGN achieves state-of-the-art performance. It ranked the 1st on the leaderboard of Argoverse benchmark on 13 Seq 2022.


% interactions. multi-agent dynamics, structured scene context and their

% 2.We propose a hierarchical lane transformer allowing for selecting the 
%      most important lanes to the target, enabling faster and equal accurate predictions.


% 3.We design a novel temporal hierarchical scene graph neural network THSGN for motion prediction.

%  Our model achieves state-of-the-art performance on the online leaderboard.  

% We propose Temporal Hierarchical Scene Graph Neural Networks (THSGN) to comine the spatial features and temporal features of the temporal traffic scenes. It 

% @



% % exploits the symmetries and the hierarchical structure in the problem of multi-agent motion prediction. 
% % In HiVT[], the traffic scene is 


% HiVT[] exploits the symmetries of the multi-agent motion prediction problem. Inspired by HiVT, 

% we propose THSGN
% .


% some mechanisms from HiVT[11] in this work for its outstanding performance. 

% @

% local encoder a local regions which is centered at one agent related to the central agent.
% Recently, vectorized representation methods are proved to be capable to capture complex interactions in traffic scenes. On the basis of it, we propose the projected vectorized representation to encode the traffic scenes

% Experiments show projected vectorized representation could understand interactions in traffic scenes better than the original method.
% @


% The projected relative position and the projected relative velocity depict how close
% two individual nodes are and how fast one node moves towards another node in
% both lateral and longitudinal direction. Compared to the relative representation, the
% projected relative representation describes the interaction between entities in a more
% detailed way, allowing downstream networks to better understand the their behavior.
% Moreover, such a projected relative representation guarantees not only translation
% invariance but also rotation invariance naturally.

% % In addition, we introduce a hierarchical lane transformer. Unlike most 
% % approaches that calculate the interaction between the agent and all lanes within a
% % certain range of the agent, the hierarchical lane transformer module can select the most
% % important lanes to the target agent, which

% %  , where they
% % first score over-sampled goal candidates and then select
% % a final set from them. However, these methods usually involve goal predictions based on sparse pre-defined anchors
% % and heuristic goal selection algorithms. In this work, we
% % propose an anchor-free and end-to-end trajectory prediction model, named DenseTNT, that directly outputs a set of
% % trajectories from dense goal candidates. 

% We evaluate THSGNNs on Argoverse forecasting benchmark. Experiments show that THSGNNs achieves the state-of-the-art performance.

% Experiments on the Argoverse motion forecasting benchmark show that our approach
% achieves state-of-the-art results. 

% % Experiments show that DenseTNT achieves state-of-the-art
% p%erformance, ranking 1st on the Argoverse motion forecasting benchmark


% Behavior prediction in dynamic, multi-agent systems is
% an important problem in the context of self-driving cars,
% due to the complex representations and interactions of road
% components, including moving agents (e.g. pedestrians and
% vehicles) and road context information (e.g. lanes, traffic
% lights). 

% This paper introduces VectorNet, a hierarchical
% graph neural network that first exploits the spatial locality
% of individual road components represented by vectors and
% then models the high-order interactions among all components. In contrast to most recent approaches, which render trajectories of moving agents and road context information as bird-eye images and encode them with convolutional neural networks (ConvNets), our approach operates
% on a vector representation. By operating on the vectorized
% high definition (HD) maps and agent trajectories, we avoid
% lossy rendering and computationally intensive ConvNet encoding steps. To further boost VectorNet’s capability in
% learning context features, we propose a novel auxiliary task
% to recover the randomly masked out map entities and agent
% trajectories based on their context. We evaluate VectorNet
% on our in-house behavior prediction benchmark and the recently released Argoverse forecasting dataset. Our method
% achieves on par or better performance than the competitive
% rendering approach on both benchmarks while saving over
% 70% of the model parameters with an order of magnitude
% reduction in FLOPs. It also outperforms the state of the art
% on the Argoverse dataset.

% Accurately predicting the future motions of surrounding
% traffic agents is critical for the safety of autonomous vehicles. Recently, vectorized approaches have dominated
% the motion prediction community due to their capability
% of capturing complex interactions in traffic scenes. However, existing methods neglect the symmetries of the problem and suffer from the expensive computational cost, facing the challenge of making real-time multi-agent motion
% prediction without sacrificing the prediction performance.
% To tackle this challenge, we propose Hierarchical Vector
% Transformer (HiVT) for fast and accurate multi-agent motion prediction. By decomposing the problem into local context extraction and global interaction modeling, our method
% can effectively and efficiently model a large number of
% agents in the scene. Meanwhile, we propose a translationinvariant scene representation and rotation-invariant spatial learning modules, which extract features robust to the
% geometric transformations of the scene and enable the
% model to make accurate predictions for multiple agents in a
% single forward pass. Experiments show that HiVT achieves
% the state-of-the-art performance on the Argoverse motion
% forecasting benchmark with a small model size and can
% make fast multi-agent motion prediction.

% Predicting the motion of multiple agents is necessary for planning in dynamic
% environments. This task is challenging for autonomous driving since agents (e.g.,
% vehicles and pedestrians) and their associated behaviors may be diverse and influence one another. Most prior work have focused on predicting independent futures
% for each agent based on all past motion, and planning against these independent
% predictions. However, planning against independent predictions can make it challenging to represent the future interaction possibilities between different agents,
% leading to sub-optimal planning. In this work, we formulate a model for predicting
% the behavior of all agents jointly, producing consistent futures that account for
% interactions between agents. Inspired by recent language modeling approaches, we
% use a masking strategy as the query to our model, enabling one to invoke a single
% model to predict agent behavior in many ways, such as potentially conditioned on
% the goal or full future trajectory of the autonomous vehicle or the behavior of other
% agents in the environment. Our model architecture employs attention to combine
% features across road elements, agent interactions, and time steps. We evaluate
% our approach on autonomous driving datasets for both marginal and joint motion
% prediction, and achieve state of the art performance across two popular datasets.
% Through combining a scene-centric approach, agent permutation equivariant model,
% and a sequence masking strategy, we show that our model can unify a variety of
% motion prediction tasks from joint motion predictions to conditioned prediction


% %TODO: Abstract




==> pages/acknowledgments.tex <==
\addcontentsline{toc}{chapter}{Acknowledgments}
\thispagestyle{empty}

\vspace*{20mm}

\begin{center}
{\usekomafont{section} Acknowledgments}
\end{center}

\vspace{10mm}

%TODO: Acknowledgments

\cleardoublepage{}


==> pages/cover.tex <==
\begin{titlepage}
  % HACK for two-sided documents: ignore binding correction for cover page.
  % Adapted from Markus Kohm's KOMA-Script titlepage=firstiscover handling.
  % See http://mirrors.ctan.org/macros/latex/contrib/koma-script/scrkernel-title.dtx,
  % \maketitle macro.
  \oddsidemargin=\evensidemargin\relax
  \textwidth=\dimexpr\paperwidth-2\evensidemargin-2in\relax
  \hsize=\textwidth\relax

  \centering

  \IfFileExists{logos/tum.pdf}{%
    \includegraphics[height=20mm]{logos/tum.pdf}
  }{%
    \vspace*{20mm}
  }

  \vspace{5mm}
  {\huge\MakeUppercase{\getFaculty{}}}\\

  \vspace{5mm}
  {\large\MakeUppercase{\getUniversity{}}}\\

  \vspace{20mm}
  {\Large \getDoctype{}}

  \vspace{15mm}
  {\huge\bfseries \getTitle{}}

  \vspace{15mm}
  {\LARGE \getAuthor{}}

  \IfFileExists{logos/faculty.pdf}{%
    \vfill{}
    \includegraphics[height=20mm]{logos/faculty.pdf}
  }{}
\end{titlepage}


==> pages/disclaimer.tex <==
\thispagestyle{empty}
\vspace*{0.8\textheight}
\noindent
I confirm that this \MakeLowercase{\getDoctype{}} is my own work and I have documented all sources and material used.

\vspace{15mm}
\noindent
\getSubmissionLocation{}, \getSubmissionDate{} \hspace{50mm} \getAuthor{}

\cleardoublepage{}


==> pages/title.tex <==
\begin{titlepage}
  \centering

  \IfFileExists{logos/tum.pdf}{%
    \includegraphics[height=20mm]{logos/tum.pdf}
  }{%
    \vspace*{5mm}
  }

  \vspace{1mm}
  {\huge\MakeUppercase{\getFaculty{}}}\\

  \vspace{5mm}
  {\large\MakeUppercase{\getUniversity{}}}\\

  \vspace{10mm}
  {\Large \getDoctype{}}

  \vspace{10mm}
  {\huge\bfseries \getTitle{} \par}

  \vspace{10mm}
  {\huge\bfseries \foreignlanguage{ngerman}{\getTitleGer{}} \par}

  \vspace{10mm}
  \begin{tabular}{l l}
    Author:          & \getAuthor{} \\
    Supervisor:      & \getSupervisor{} \\
    Advisor:         & \getAdvisor{} \\
    Submission Date: & \getSubmissionDate{} \\
  \end{tabular}

  \IfFileExists{logos/faculty.pdf}{%
    \vfill{}
    \includegraphics[height=20mm]{logos/faculty.pdf}
  }{}
\end{titlepage}

